Adaptive Model Predictive Control by Learning Classifiers

Stochastic model predictive control has been a successful and robust control framework for many robotics tasks where the system dynamics model is slightly inaccurate or in the presence of environment disturbances. Despite the successes, it is still unclear how to best adjust control parameters to the current task in the presence of model parameter uncertainty and heteroscedastic noise. In this paper, we propose an adaptive MPC variant that automatically estimates control and model parameters by leveraging ideas from Bayesian optimisation (BO) and the classical expected improvement acquisition function. We leverage recent results showing that BO can be reformulated via density ratio estimation, which can be efficiently approximated by simply learning a classifier. This is then integrated into a model predictive path integral control framework yielding robust controllers for a variety of challenging robotics tasks. We demonstrate the approach on classical control problems under model uncertainty and robotics manipulation tasks.

==> header.tex <==
%\usepackage[most]{tcolorbox}
% \usepackage{algorithmic}

\usepackage{makecell}
\usepackage{amsfonts}
%\usepackage[inline]{enumitem}
\usepackage{amsmath}
\usepackage{amsopn}
\usepackage{amssymb}  %
\usepackage{bm}
\usepackage{array}
\usepackage{bold-extra}
\usepackage{braket}
\usepackage{calligra}
\usepackage{epstopdf}
\usepackage{float}
\usepackage{graphicx,epstopdf}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{lipsum}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\usepackage{pgfplots}
\usepackage{pifont}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{wrapfig}
\usepackage{xspace}
%\usepackage[noabbrev,capitalise]{cleveref}

\usepackage{paralist}

\usepackage{times}


\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{natbib}
\usepackage{graphicx}
\usepackage{url}
%\usepackage{algorithm2e}


% \edef\tmp{\pgfmathresult}
% \pgfkeys{/pgf/fpu=false}
% \pgfkeys{/pgf/fpu}
% \pgfmathparse{16383+1}
% \pgfplotsset{compat=1.12}
% \pgfplotstableset{col sep=comma}
% \tikzexternalize[prefix=cached_figures/, mode=list and make]
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc,patterns,angles,quotes}
\usetikzlibrary{external}
\usetikzlibrary{pgfplots.groupplots}
\colorlet{texcscolor}{blue!50!black}
\colorlet{texemcolor}{red!70!black}
\colorlet{texpreamble}{red!70!black}
\colorlet{codebackground}{black!25!white!25}



%%%% custom macros

\newcommand{\x}{x}
\newcommand{\ix}{x}
\newcommand{\iy}{{y}}
\newcommand{\ip}{{p}}
\newcommand{\iq}{{q}}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\originalvf}{\tilde f}
\newcommand{\ltwonorm}[1]{\|#1\|_2}
\newcommand{\coloneqq}{:=}
\newcommand{\metricsup}[2]{\|#1\|_{#2}}
\newcommand{\metricdyn}[3]{d_{#2, #3}(#1)}
\newcommand{\generalineq}{\unrhd}
\newcommand{\poly}[1]{\mathcal P_{#1}}
\newcommand{\SETALG}{\Lambda}
  
% path to images
%\graphicspath{ {./img/} }



\newcommand{\NINTERPOLATION}{\operatorname{{\bf Interp}}}
\newcommand{\NPOS}{\operatorname{{\bf Pos}}}
\newcommand{\NMON}{\operatorname{{\bf Mon}}}
\newcommand{\NINV}{\operatorname{{\bf Inv}}}
\newcommand{\NGRAD}{\operatorname{{\bf Grad}}}
\newcommand{\NHAMILTONIAN}{\operatorname{{\bf Ham}}}
\newcommand{\NSYM}{\operatorname{{\bf Sym}}}

  
\newcommand{\INTERPOLATION}[1]{\NINTERPOLATION(#1)}
\newcommand{\POS}[1]{\NPOS(#1)}
\newcommand{\MON}[1]{\NMON(#1)}
\newcommand{\INV}[1]{\NINV(#1)}
\newcommand{\GRAD}{\NGRAD}
\newcommand{\HAMILTONIAN}{\NHAMILTONIAN}
\newcommand{\SYM}[1]{\NSYM(#1)}


\newcommand{\LS}{{L_{S,\Omega}}}
\newcommand{\LiS}[1]{{L_{S_{#1},\Omega}}}

\newcommand{\CD}{{C_1^{\circ}(\Omega)}}


\newtheorem{mydef}{Definition}
\newtheorem{myexp}{Example}
\newtheorem{myremark}{Remark}
\usepackage[shortlabels]{enumitem}
%\usepackage{enumitem}

% \setlist{leftmargin=.5mm}

% \usepackage{titlesec}
% \titlespacing*{\section} {0pt}{6pt}{2pt}
% \titlespacing*{\subsection} {0pt}{6pt}{2pt}


\pgfplotsset{compat = 1.3}
% \titlespacing*{\subsection}
% {0pt}{5.5ex plus 1ex minus .2ex}{4.3ex plus .2ex}





%% Code style
\usepackage{listings}
\definecolor{commentgreen}{RGB}{2,112,10}
\definecolor{eminence}{RGB}{108,48,130}
\definecolor{weborange}{RGB}{255,165,0}
\definecolor{frenchplum}{RGB}{129,20,83}
\lstdefinestyle{JuliaListing}{
  language=Python,
  basicstyle=\small,
  numbers=none,
  stepnumber=1,
  numbersep=10pt,
  tabsize=4,
  showspaces=false,
  showstringspaces=false,
  commentstyle=\color{commentgreen},
  keywordstyle=\color{eminence},
  otherkeywords={@variable,@objective,@constraint,@polyvar},
  frame=tb,
  mathescape=true,
  escapechar=\%,
  captionpos=b,
}
\newcommand*{\CodeComment}[2][5.0cm]{\hfill\makebox[#1][l]{\textcolor{commentgreen}{\#
      #2}}}
\renewcommand{\lstlistingname}{Source Code}% Listing -> Algorithm

% \let\cite\citep
% \usepackage{jlcode}

  


